On Invariance, Equivariance, Correlation and Convolution of Spherical Harmonic Representations for Scalar and Vectorial Data

The mathematical representations of data in the Spherical Harmonic (SH) domain has recently regained increasing interest in the machine learning community. This technical report gives an in-depth introduction to the theoretical foundation and practical implementation of SH representations, summarizing works on rotation invariant and equivariant features, as well as convolutions and exact correlations of signals on spheres. In extension, these methods are then generalized from scalar SH representations to Vectorial Harmonics (VH), providing the same capabilities for 3d vector fields on spheres

==> feature_lbp.tex <==
\cleardoublepage
\chapter{\label{sec:feature:LBP}LBP Features}

``Local Binary Pattern'' (LBP) \cite{LBP} have been established as a standard feature based method
for 2D image analysis. LBP have been successfully applied to a wide range of different applications from
texture analysis \cite{LBP} to face recognition \cite{face}.
Various extensions to the basic LBP algorithms were published in recent years, including
rotation invariant binary pattern (rLBP) and computationally efficient ``uniform binary pattern'' (uLBP) - a comprehensive overview
can be found in \cite{LBP}.\\

In this chapter, we extend the original LBP from 2D images to 3D volume data and generalize the rotation invariant
rLBP \cite{3Dlbp} and uLBP \cite{3Dulbp}, implementing full rotation invariance in 3D.

\paragraph{Related Work:} So far, standard LBP have only been applied to 2D images and 2D time series. There are several recent
publications on ``volume local binary patterns'' (vLBP)\cite{VLBPpami}\cite{VLBPeccv}\cite{VLBPmva}, but confusingly these methods
deal with dynamic texture analysis on 2D time series and not on full 3D volumetric data. Accordingly, vLBP only provide
invariance towards rotations around the z-axis.

\section{\label{sec:feature:LBP2D}LBP in 2D.} 
In contrast to most of the other feature methods we discuss in this thesis, ``Local Binary Pattern'' are defined in a discrete setting
 and operate directly on a pixel/voxel grid.
LBP encode $N$ neighboring points with gray values $u_i, i\in\{0\dots N-1\}$ in relation to the
center pixel. In 2D, these neighbors are given as equidistant points on a circle with radius $r$ around a center pixel with gray value $c$
(see Fig. \ref{fig:feature:LBPscheme}):  
\begin{eqnarray}
\label{eq:feature:LBPeq}
\mathrm{LBP}_N^r := \sum_{i=0}^N \mathrm{sig}(u_i - c) \cdot 2^i \\
\text{with } \mathrm{sig}(x) :=
\left\{
\begin{matrix}
1 & \text{\quad\quad for } x>0\\
0  & \text{\quad\quad otherwise}
\end{matrix}
\right.\nonumber
\end{eqnarray}
The center is usually chosen to be located at pixel/voxel positions, while the gray-values of the
sampling points are obtained via interpolation.\\
The binarization of the gray-value relations by $\mathrm{sig}(x)$ makes LBPs invariant towards monotonic gray-scale changes and the 
weighting with powers of two guarantees a unique coding. 
For more details on 2D LBP refer to \cite{LBP}.
\begin{figure}[htp]
\centering
\psfrag{c}{\footnotesize $c$}
\psfrag{x0}{\color{white}\footnotesize $u_0$}
\psfrag{x1}{\color{white}\footnotesize $u_1$}
\psfrag{x2}{\color{white}\footnotesize $u_2$}
\psfrag{x3}{\color{white}\footnotesize $u_3$}
\psfrag{x4}{\color{white}\footnotesize $u_4$}
\psfrag{x5}{\color{white}\footnotesize $u_5$}
\psfrag{x6}{\color{white}\footnotesize $u_6$}
\psfrag{x7}{\color{white}\footnotesize $u_7$}
\psfrag{sum}{\large $\sum\limits_i \mathrm{sig}(u_i - c)\cdot 2^i$}
\psfrag{sig}{$\mathrm{sig}(u_i - c)$}
\includegraphics[width=0.3\textwidth]{FIGURES/LBP.eps}
\caption{\label{fig:feature:LBPscheme} Computation of a 2D LBP with $N=8$ sampling points with gray-values $u_i$ around the center pixel 
with gray-value $c$.}
\end{figure}

\subsection{Rotation Invariance in 2D}
\index{rLBP}
It is easy to realize that the naive implementation (\ref{eq:feature:LBPeq}) of LBPs is not rotation invariant. To overcome this drawback,
\cite{LBP} introduced a refined version of the initial formulation which achieves invariance via normalization:
\begin{eqnarray}
\label{eq:feature:rLBP}
\mathrm{rLBP}_N^r &:=& \min\left(\mathrm{ROT}(LBP_N^r, n)\right)\\
&&\text{with } n=0\dots N-1,\nonumber
\end{eqnarray}
where $\mathrm{ROT}(LBP_N^r, n)$ is a discrete rotation of the assignment of the neighbors $u_i$ to the powers of two $2^{i+n}$ by $n$ steps. 
In 2D, this can be implemented via cyclic shifts:
\begin{eqnarray}
\label{eq:feature:rLBP2D}
\mathrm{rLBP}_N^r &:=& \min\left(\sum\limits_i \mathrm{sig}(u_i - c)\cdot 2^{(i+n)\mod N} \right)\\
&&\text{with } n=0\dots N-1,\nonumber
\end{eqnarray}

More details on rotation invariant 2D LBP can be found in \cite{LBP}.

\section{\label{sec:feature:uLBP}Uniform Local Binary Patterns (uLBP) in 2D}
\index{uLBP}
One commonly used extension of LBPs are the so called ``uniform'' LBPs (uLBP), which were introduced in \cite{ulbp}. The uLBPs form
a subset of all theoretically possible patterns, which is restricted to LPBs with a ``non-uniformity'' measure $U(LBP_N^r) \leq 2$. 
The ``non-uniformity'' measure is defined as the number of $0-1$ and $1-0$ transitions in the cyclic sequence 
$\{\mathrm{sig}(u_i - c)|i=0,\dots,N\}$.
Experiments have shown that up to 90\% of all 2D patterns belong to this subset \cite{ulbp}.
Fig. \ref{fig:feature:uLBPscheme} shows a set of uLBP templates.\\
\begin{figure}[htp]
\centering
\includegraphics[width=0.5\textwidth]{FIGURES/uLBP.eps}
\caption{\label{fig:feature:uLBPscheme} Template classes for uniform LBPs using $N=8$ sampling points around the center $c$. Black points 
correspond to the binary value $0$, gray to $1$.}
\end{figure}
Practically, the uLBP method performs a rotation invariant template matching by simply ``counting'' the number of ones and rejecting
input signals with $U(LBP_N^r) > 2$. The number of ones is then used to encode the pattern as uLBP.\\
Due to this template nature, uLBPs are easier to extend to 3D volume data - an approach we are following in section \ref{sec:feature:uLBP}, 
but first, we will discuss the problems of a ``naive'' LBP implementation in 3D.

\section{\label{sec:feature:LBP3D}Naive Implementation of LBP in 3D}
\index{Naive 3D LBP}
At a first glimpse, the extension of LBPs to 3D seems to be straightforward: Simply pick a center voxel with gray value $c$,
and sample a fixed number of $N$ equidistant points with gray values $x_0 \dots x_{N-1}$ on the respective sphere with radius $r$.
Compute $\mathrm{sig}(u_i - c)$ for all $u_i$ and encode the binary pattern as in the usual LBP algorithm.\\
This appears to be very simple, but one has to face several severe problems following  this direct approach:
first, equidistant sampling on a sphere is a very hard
task which is known as {\it Fejes Toth's} problem \cite{sampling}. 
In general, it cannot be solved analytically. Since we need equidistant sampling
in order to achieve full rotation invariance, we are limited to the few known point sets where a sampling is known \cite{sampling} or
we have to use rather expensive numerical approximations.
Secondly, rotation invariant LBPs require an ordering of the sampled points, which is trivial in 2D - but turns out to be a quite hard
problem given three degrees of freedom on a sphere.
And last, computational complexity becomes an issue with the vastly rising number of sampling points needed on a
sphere.\\

To cope with these problems we utilize some of the techniques introduced in chapter \ref{sec:feature:mathbg} and \ref{sec:feature:SH} to
derive methods for the computation of LBPs in the harmonic domain. This way, we are able to avoid the sampling and ordering problems 
at significantly reduced computational complexity.\\
First we give a 3D extension for uLBPs \cite{3Dulbp} which has its limitations and should be seen as preliminary work to our later
general extension of LBPs for 3D volume data \cite{3Dlbp}.  



\newpage
%--------------------------------------
% fuLBP
%-------------------------------------
\section{\label{sec:feature:uLBP3D}Fast 3D uLBP (fuLBP)}
\index{LBP Features}\index{fuLBP}\index{3D uLBP}
We presented a first approach towards 3D rotation invariant LBPs in form of a generalization of uniform LBPs (see section 
\ref{sec:feature:uLBP}) in \cite{3Dulbp}. \\
This method should be seen as preliminary work to our later
general extension of LBPs for 3D volume data (see section \ref{sec:feature:LBPfast3D}). It demonstrates that it is possible to engage
the computation of 3D LBPs in the harmonic domain. Hence, we do not endorse the practical usage of this approach - it should been seen
as proof of concept which contributes some important ideas for the methods introduced in section \ref{sec:feature:LBPfast3D}.
\subsection{Feature Design}
The key idea of the ``fast 3D uLBP'' (fuLBP) is rather simple: we redefine the uLBP algorithm as simple template matching problem.
Given all uniform patterns ${\bf uLBP}_i^r$ with radius $r$, 
we search for the best match with the underlying data. In the 2D case, this matching is performed by simply 
counting the ``ones'' after the binarization step $\mathrm{sig}(x)$ (see section \ref{sec:feature:uLBP}).\\
As pointed out in section \ref{sec:feature:LBP3D}, such a direct approach would be too expensive in a 3D application. Therefore we 
suggest to perform the template matching in the harmonic domain. In order to do so, we need several things: 
first, we define the uniform pattern templates as ${\bf uLBP}_i^r: S^2\times\{0,1\} \rightarrow \{0,1\}$. Secondly, we compute 
the Spherical Harmonic
expansions (\ref{eq:feature:SHcoeff}) ${\cal SH}\big(X|_{S[r]({\bf x})}\big)$ of the local shperical neighborhood of ${\bf x}$ in $X$  and 
${\cal SH}[r]({\bf uLBP}_i^r)$
of the ``uniform patterns''. Thirdly, we need to be able to perform the binarization in the harmonic domain, and finally, we need a 
similarity measure.
\subsection{Theory}
The first step is trivial: we obtain ${\cal SH}\big(X|_{S[r]({\bf x})}\big)$ and ${\cal SH}[r]({\bf uLBP}_i^r)$ directly via the Spherical 
Harmonic forward transformation (\ref{eq:feature:SHforward}). The binarization step is more difficult:

\paragraph{Binarization:}
Since it is impossible to perform a local binarization at sampling points $u_i$ after we have transformed the data into frequency space, 
we reduce the sparse binarization $\mathrm{sig}(u_i-c)$ to the continuous subtraction of $c$ at all points of 
${\cal SH}[r](X)({\bf x})$. 
We subtract the value at the center $c=X({\bf x})$ from the signal expanded in ${\cal SH}\big(X|_{S[r]({\bf x})}\big)$. 
In the original setting,
$c$ is constant for all evaluations of $\mathrm{sig}(u_i-c)$, hence, the subtraction is equal to a
shift of the constant component on ${\cal SH}\big(X|_{S[r]({\bf x})}\big)$ and thus only effects the $0$th coefficient:
\begin{eqnarray}
\label{eq:feature:SHbinarize}
\left({\cal SH}\big(X|_{S[r]({\bf x})}\big)-X({\bf x})\right)^0_0 := \left({\cal SH}\big(X|_{S[r]({\bf x})}\big)\right)^0_0 - 
(X({\bf x})\cdot b_{abs}),
\end{eqnarray}
where $b_{abs}$ is the absolute number of expansion bands. All other coefficients with $l>0, -l\leq m \leq l$ are not effected:
\begin{eqnarray}
\left({\cal SH}\big(X|_{S[r]({\bf x})}\big)-X({\bf x})\right)^l_m := \left({\cal SH}\big(X|_{S[r]({\bf x})}\big)\right)^l_m.
\end{eqnarray}

\paragraph{Similarity Measure:}
Finally, we need a rotation invariant similarity measure for the actual template matching. In \cite{3Dulbp}, we suggested to use the
${\cal SH}_{abs}$ measure from section \ref{sec:feature:SHabs}. ${\cal SH}_{abs}$ is easy to implement and very fast since we are already
operating in the harmonic domain. But, as pointed out in section \ref{sec:feature:SHabs}, ${\cal SH}_{abs}$ is not very discriminative. 
Hence,
we also might use the fast correlation from section \ref{sec:feature:shcorr} which provides more discrimination power at the cost of higher
computational complexity.

\subsection{Implementation}
The implementation of the fuLBP is straightforward. We follow the implementation of the Spherical Harmonic transformation as described in
section \ref{sec:feature:implement}. Details on the implementation of the similarity measures can be found in section \ref{sec:feature:SHabs}
and \ref{sec:feature:sincinterpol} respectively.

\paragraph{Multi-Channel Data:} fuLBPs cannot directly combine data from several channels into a single feature. In case of multi-channel 
data, we would have to separately compute features for each channel.

\paragraph{Complexity:}
The main argument for the harmonic approach, besides the fact that we can avoid the equidistant sampling problem, is the 
better computational complexity.
If we assume that we need to extract the features at each of the $m$ voxels of the input volume $X$,  have $H$ ``uniform patterns'',
and take $N$ samples, the naive implementation of $uLBP_N^r$ has a complexity of $O(m\cdot N^2 \cdot H)$, 
where $N$ samples have to be evaluated at all $m$ points and finding 
the right pattern takes another $O(N\cdot H)$. The harmonic approach $fuLBP_N^r$ lies in $O\left((m \log m)\cdot b_{\max}^2  + 
m\cdot H\cdot b_{\max}^2\right)$: 
$O(m \log m)$ for the Fourier transform of $b_{\max}^2$ bands plus the
cost of finding the right of $H$ possible pattern. Hence, the computation complexity in the harmonic domain does not directly dependent 
on the number of samples. In 3D, where $N>>b_{\max}$, the additional overhead for the Fourier transform will drastically pay off.
\paragraph{Parallelization:} Further speed-up can be achieved by parallelization (see section \ref{sec:feature:parallelization}): 
the data can be transformed into
the harmonic domain by parallel computation of the coefficients and the computation at each voxel can also be split into several threads.
For ${\cal C}$ CPU cores with ${\cal C}\leq b_{\max}^2$ and ${\cal C}\leq m$ we obtain:
$$O((m \log m) \cdot \frac{b_{\max}^2}{\cal C}) +O( \frac{m}{\cal C}\cdot H\cdot b_{\max}^2)$$

\subsection{Discussion}
At first glimpse, fuLBPs appear to be quite attractive since the two major problems of a naive implementation are solved sufficiently: 
the equidistant sampling problem and the complexity. But there is an additional general problem concerning a 3D extension of uLBPs: the
definition of 3D ``uniform patterns''.\\
It is clear that the 2D definition by $U(LBP_N^r) \leq 2$ (see \ref{sec:feature:uLBP}) is not applicable in the 
3D case with its ($\Phi, \Theta$)-coordinate system on the 2-Sphere (see section \ref{sec:feature:shrot}). But how should the ``uniform 
patterns'' be 
chosen, regarding the fact that the number of patterns $H$ has a large impact on the complexity? \\
In \cite{3Dulbp}, we suggested to generate a data dependent set of ``uniform patterns'' via clustering of training data to overcome
this problem. Such a ``codebook'' approach makes sense in cases where the number of codebook entries can be kept small - which strongly 
depends on the individual problem and is in fact a strong limitation of the entire fuLBP concept. 


\newpage
%-----------------------------------
% fLBP
%----------------------------------
\section{\label{sec:feature:LBPfast3D}Fast 3D LBP (fLBP)}
\index{LBP Features}\index{fLBP}\index{3D LBP}
After the introduction of fuLBPs \cite{3Dulbp} (see section \ref{sec:feature:uLBP3D}) we presented a general LBP extension  
to 3D volume data in \cite{3Dlbp}, which we named fLBP. Both methods have in common that we are following the key idea of a template formulation \cite{3Dulbp}.
Hence, we first reformulate the general LBPs as template matching problem. Refere to section \ref{sec:feature:LBP2D} for the original 
formulation.

\subsection{Feature Design}
The template approach is based on the pre-computation of so-called ``\textbf{2-patterns}''. A 2-pattern $P^r_N$ is the volume representation
(3D grid) of a set of $N$ equidistant points on a sphere with radius $r$.
Each of theses points is weighted in an arbitrary but fixed order with the gray values $p_0:=2^0,\dots,p_{N-1}=2^{N-1}$. All other points in
the volume are set to zero.\\
For each LBP computation at ${\bf x}$ in $X$, we consider the local spherical neighborhood around ${\bf x}$ 
$S[r]({\bf x}) := \{{\bf x}_i \in \mathbb{R}^n | \|{\bf x}-{\bf x}_i\|=r\}$ with radius $r$. 
Given a center point with gray value $c=X({\bf x})$, we compute the point-wise threshold $T$ of the entire volume grid:
\begin{equation}
\forall {\bf x}_i \in S[r]({\bf x}): \text{\quad} T[r,{\bf x}]({\bf x}_i) :=\mathrm{sig}\big(X\big|_{S[r]({\bf x})}({\bf x}_i) - c\big).
\end{equation}
The resulting LBP is then computed via the dot-product of the 2-pattern and the threshold:
\begin{equation}
\mathrm{LBP}_N^r(X,{\bf x}) := \langle P^r_n , T[r,{\bf x}]\rangle.
\end{equation}
Hence, given an equidistant sampling, the computation of 3D LBP with the template approach is not so difficult - 
the actual problem is to obtain rotation invariance in 3D.

\subsubsection{Rotation Invariance}
In the 2D case, where rotations have only one degree of freedom, invariance can be realized via minimum search over all cyclic
shifts of the
circular 2-pattern in $O(N)$ \eqref{eq:feature:rLBP}. Using our fixed 2-pattern on a sphere, we encounter three degrees of freedom.
This makes the 3D case a lot more difficult and computationally expensive.\\
We engage this problem by revising \eqref{eq:feature:rLBP}:
we can reformulate the problem as the computation of the minimum of the full correlation ($\#$) over all angles
of the fixed 2-pattern template $P^N_r$ with $T[r,{\bf x}]$:
\begin{equation}
\mathrm{rLBP}_N^r := \min(P_N^r \# T[r,{\bf x}]).
\label{eq:feature:fLBPfinal}
\end{equation}
Given our fast correlation in the harmonic domain (see section \ref{sec:feature:shcorr}), 
we compute the rotation invariant fLBP in three steps: first, generate the 2-pattern $P^r_N$ and compute $T[r,{\bf x}]$ using known
equidistant samplings \cite{sampling} with 24 to 124 samples. Then expand both
in Spherical Harmonics and obtain the coefficients $\widehat{P^r_N}$ and $\widehat{T[r,{\bf x}]}$. Finally, compute the rLBP via 
the minimum of the fast correlation of $\widehat{P^r_N}$ and $\widehat{T[r,{\bf x}]}$ as stated in (\ref{eq:feature:fLBPfinal}).

\subsection{\label{sec:feature:fLBPthres}Implementation}
The actual bottleneck of our approach is the complexity of the computation of $T[r,{\bf x}]$ which is increasing with the number of
sampling points. For full gray-scale invariance we have to compute $T[r,{\bf x}]$ correctly, 
but there is an elegant way to approximate $\widehat{T[r,{\bf x}]}$ 
while preserving a gray-scale robustness: we compute $\widehat{S[r]({\bf x})}$ and subtract $c=X({\bf x})$ in the frequency domain, 
which only affects the 0th coefficient $\widehat{T[r,{\bf x}]}$ (\ref{eq:feature:SHbinarize}).
Hence, we no longer have a binary but continuous weighting of the n-pattern. 

\paragraph{Multi-Channel Data:} fLBPs can only combine data from two different channels into a single feature. We can set the center point to
the first channel, and then sample the neighborhood from the second channel.

\subsubsection{Complexity}
The overall complexity for the evaluation of $fLBP$ at all $m$ voxels of $X$ is:
$$ O( (m \log m) \cdot b_{\max}^2 + m \cdot (N + (b_{\max}^2+p) \log (b_{\max}^2+p)))$$
Where $O( (m \log m) \cdot b_{\max}^2)$ is the cost for the Spherical Harmonic transform with $b_{\max}$ expansion bands, 
$O( m \cdot (b_{\max}^2+p) \log (b_{\max}^2+p))$ the cost of the fast correlation with padding $p$ (see section \ref{sec:feature:shcorr}) 
and $O(N)$ the thresholding for $N$ sampling points.\\
The dominating cost factor is the number of sampling points $N$, since $N>>b_{\max}$. If we use the approximation of the threshold 
from section \ref{sec:feature:fLBPthres}, the costs become independent of $N$: 
$$ O( (m \log m) \cdot b_{\max}^2 + m \cdot ((b_{\max}^2+p) \log (b_{\max}^2+p)))$$

\paragraph{Parallelization:} Further speed-up can be achieved by parallelization (see section \ref{sec:feature:implement}): the data can be transformed into
the harmonic domain by parallel computation of the coefficients and the computation at each voxel can also be split into several threads.
For ${\cal C}$ CPU cores with ${\cal C}<b_{\max}^2$ and ${\cal C}<m$ we obtain:
$$ O( (m \log m) \cdot \frac{b_{\max}^2}{\cal C}) + O(\frac{m}{\cal C} \cdot ((b_{\max}^2+p) \log (b_{\max}^2+p))$$
\subsection{Discussion}
The presented generalization of the LBP feature for 3D volume data preserves all favorable properties of the original 2D formulation at considerable 
complexity. If we neglect exact thresholding, fLBPs can be computed very fast. 




==> feature_selection.tex <==
\cleardoublepage
\chapter{\label{sec:feature:featureselect}Feature Selection}
\index{Feature Selection}
Basically all the features we have introduced in the previous chapters take some parameters like radius, maximum expansion band or
non-linear mappings $\kappa_i$. The correct selection of these parameters is absolutely vital to the feature performance.\\
While it is possible to use some a-priori knowledge and expert experience to set some of the parameters, i.e. the radius, it is in most
cases not possible to determine the other parameters directly. Therefore, we apply automatic feature selection methods that use
labeled training samples to determine the most discriminative features.\\

We distinguish between two different types of feature selection methods: first, the class of {\bf combinatorial} algorithms. These
generic selection algorithms are most common in literature. Basically, they perform an ``intelligent'' combinatoric
search over all possible feature combinations. This is more or less a ``brute force'' approach, where we have to compute all 
features and search the best combination. For this purpose, we use two different methods, MMD \cite{MMD} and SIMBA \cite{SIMBA} which are well known from literature.\\
For some features, like $np$- and $nv$-Features, the parameter space is simply to large for even the smartest combinatoric search: it
is simply not feasible to compute all possible features. For these cases, we introduce the second class of specialized (feature dependent) 
{\bf constructive} data driven feature selection methods which use labeled training samples to actually learn the best feature parameters. 

\paragraph{Structure:} The remainder of this chapter is structured as follows: first, before we review the two combinatoric feature selection 
methods MMD (section \ref{sec:feature:featureselect_mmd}) and SIMBA (section \ref{sec:feature:featureselect_simba}), we state
basic mathematical definitions which found the basis for both methods.\\
Then, we introduce and derive our constructive feature selection algorithm for $np$- and $vp$-Features in section 
\ref{sec:feature:select_data}. 


\subsection{\label{sec:feature:featureselect_BG}Mathematical Background}
\index{Feature Selection}
Given two random variables $X$ and $Y$ with marginal probabilities $p_1(x), p_2(x)$ and the joint probability distribution $p(x,y)$,
we define the following  terms:

\paragraph{Mutual Information:} of two random variables is a quantity that measures the mutual dependence of the two variables:
\begin{equation}
\label{eq:feature:select_muatualinformation}
I(X;Y) := \sum\limits_{y\in Y}\sum\limits_{x\in X} p(x,y) \log{\frac{p(x,y)}{p_1(x)p_2(y)}}.
\end{equation}

\paragraph{Kullback-Leibler Divergence:} is a non-commutative measure of the difference between two probability distributions P and Q:
\begin{equation}
\label{eq:feature:select_kl}
KL(P\|Q)
:= \sum\limits_i P(i) \log{\frac{P(i)}{Q(i)}}.
\end{equation}


\section{\label{sec:feature:featureselect_mmd}Maximum Marginal Diversity (MMD)}
\index{Feature Selection}\index{Maximum Marginal Diversity (MMD)}
The first of the two combinatoric feature selection algorithms we choose to apply for several of our problems (see part III) is the Maximum 
Marginal Diversity (MMD) approach by \cite{MMD}. 
MMD is fast, easy to implement and under certain constraints, MMD is able to compute the best $n$ features in a minimum Bayesian
error sense by applying the {\bf Infomax Principle} \cite{infomax}.\\ 

\paragraph{Infomax Principle:} For classification problems, Infomax \cite{infomax} endorses the selection of features that maximize 
the mutual information between features and class labels:\\

{\bf Lemma:} {\it Given a classification problem (see section \ref{sec:learning:intro}) with $m$ classes and features ${\bf X} := T({\bf Z})$ which are 
drawn from the random variables (input data) $\bf Z$, then the best feature space is the one that maximizes the mutual information 
$I(Y;{\bf X})$} \cite{infomax}.\\  

It has been shown in \cite{MMD}, that the Infomax solution of a problem is in fact a very close approximation of the Bayesian Error 
estimate of 
this classification problem. However, it is very hard to actually compute an Infomax solution without searching the all possible feature 
combinations or using numerical approximations.\\
One way to overcome this problem was also introduced in \cite{MMD}, where it has been observed that Infomax emphasizes solutions with large 
marginal diversities.

\paragraph{Marginal Diversity (MD):}
Given a classification problem (see section \ref{sec:learning:intro}) with features ${\bf X} = (X_1,\dots,X_n)$, the Marginal Diversity (MD)
for a single feature $X_k$ is given by the divergence of the probability densities for single classes $P_{X_k|Y}(x|i)$ with all classes:
\begin{equation}
\label{eq:feature:select_md}
md(X_k) := \langle KL(P_{X_k|Y}(x|i)\|P_{X_k}(x)\rangle_Y.
\end{equation}

\subsection{Feature Selection with the Maximum Marginal Diversity (MMD)}
Using the Marginal Diversity formulation (\ref{eq:feature:select_md}), \cite{MMD} was able to show that in cases where the knowledge of the
class label does not change the mutual information between the features, selecting features of maximal marginal diversity results in the same 
solution as the Infomax algorithm.\\

Following these results, \cite{MMD} also introduced a very simple and easy to implement algorithm for computation of the MMD, which
uses histogram approximations of the probability densities:

\begin{algorithm}
\caption{MMD feature selection}
\label{algo:feature:mmd}
\begin{algorithmic}
\FORALL{features $X_k$ with $k \in\{1,\dots,n\}$}
\FORALL{labels $i \in \{1,\dots,m\}$}
\STATE compute the histogram $h_{k,i}$ of $P_{X_k|Y}(x|i)$
\ENDFOR
\STATE compute $h_{k} = 1/m\sum\limits_i h_{k,i}$
\ENDFOR
\STATE compute $md(X_k) = \sum\limits_i p_i {\bf h}_{k,i}^T \log{{\bf h}_{k,i}}/h_{k}$
\STATE sort $X_k$ by $md(X_k)$
\STATE RETURN top $N$ $X_k$
\end{algorithmic}
\end{algorithm}

The main advantage of the MMD algorithm is that it is able to perform the Infomax approximation of $n$ features in $O(n)$.

\subsection{\label{sec:feature:featureselect_mmd_disscuss}Discussion}
The Maximum Marginal Diversity algorithm is easy to implement and provides an accurate and fast approximation of the Infomax principle.
However, the fact that MMD treats all features independently can cause some unexpected drawbacks in the quality of the selected features: 
in cases (and the nature of our features endorses theses cases) where two or more features are redundant, MMD will rank 
all features the same - even though just one of these features would provide the same separability properties as all of them together.\\
This behavior makes it very hard to decide how many features are actually needed and causes the risk to neglect generally weaker features 
which actually would provide additional information. Hence,  MMD only provides the best individual features, but not the best feature combination. 


\section{\label{sec:feature:featureselect_simba}SIMBA}
\index{Feature Selection}\index{SIMBA}
We try to overcome the shortcomings of the MMD algorithm (see \ref{sec:feature:featureselect_mmd_disscuss}) with a second feature selection 
method: the so-called SIMBA approach \cite{SIMBA}.\\
SIMBA uses an iterative search over the possible feature combinations in order to find the best feature combination. Hence, SIMBA does not
have the same problems as MMD, but we have to expect a higher computational complexity.\\

While there are numerous other feature selection methods which apply smart combinatoric search strategies, we have chosen SIMBA because it 
utilizes a 
maximum margin measure to evaluate the quality of feature combinations. This is a natural choice, since we are applying maximum
margin classifiers, i.e. support vector machines (SVM), later on (see chapter \ref{sec:learning:svm}).\\

While SVMs optimize the {\bf sample-margin}, i.e. the distance between the instances and the decision boundary (see chapter 
\ref{sec:learning:svm} for details), 
\cite{SIMBA} showed that a lower bound to the sample-margin is given by the much easier to compute {\bf hypothesis-margin} 
$\Theta_P({\bf x})$ (\ref{eq:learning:simba_dist}). Given a set of points $P$ and the feature vector ${\bf x}$, 

\begin{equation}
\Theta_P({\bf x}) := \frac{1}{2}\big(\|{\bf x}-nearmiss({\bf x})\| - \|{\bf x}-nearhit({\bf x})\|\big),
\label{eq:learning:simba_dist}
\end{equation}
where $nearmiss({\bf x})$ and $nearhit({\bf x})$ denote the nearest points in $P$ with a different/same class label.\\ 

Using this definition of the margin, \cite{SIMBA} introduce a weighting ${\bf w}$ of the individual features, such that:
\begin{eqnarray}
\Theta_P^{\bf w}({\bf x}) &:=& \frac{1}{2}\big(\|{\bf x}-nearmiss({\bf x})\|_{\bf w} - \|{\bf x}-nearhit({\bf x})\|_{\bf w}\big)\\
&& \text{with } \|z\|_{\bf w} := \sqrt{\sum\limits_i {\bf w}_i^2 z_i^2}.\nonumber
\label{eq:learning:simba_distweight}
\end{eqnarray}
Given such a weighting, \cite{SIMBA} use a leave one out (LOO) (see section \ref{sec:learning:learning}) strategy to compute the quality 
of the margin induced by a set $S$ of features with weights ${\bf w}$:

\begin{equation}
e({\bf w}) := \sum\limits_{{\bf x}\in S}\Theta^{\bf w}_{S\setminus {\bf x}}({\bf x}).
\label{eq:learning:simba_energy}
\end{equation}
In order to apply a gradient decent algorithm for the iterative search of the best feature weighting, one differentiates (\ref{eq:learning:simba_energy}):
\begin{eqnarray}
(\bigtriangledown e({\bf w}))_i &:=& \frac{\partial e({\bf w})}{\partial {\bf w}_i}\\
&=& \sum\limits_{{\bf x}\in S} \frac{\partial\Theta({\bf x})}{\partial {\bf w}_i}\nonumber\\
&=&\frac{1}{2}\sum\limits_{{\bf x}\in S}\big(\frac{({\bf x}_i-nearmiss({\bf x})_i)^2}{\|{\bf x}-nearmiss({\bf x})\|_{\bf w}}-\frac{({\bf x}_i-
nearhit({\bf x})_i)^2}{\|{\bf x}-nearhit({\bf x})\|_{\bf w}}\big){\bf w}_i.\nonumber
\label{eq:learning:simba_gradient}
\end{eqnarray}
Based on this gradient formulation, \cite{SIMBA} derived an easy to implement and reasonably fast algorithm for maximum margin feature 
selection called SIMBA (see algorithm \ref{algo:feature:simba}).

\begin{algorithm}
\caption{SIMBA feature selection}
\label{algo:feature:simba}
\begin{algorithmic}
\STATE initialize ${\bf w}=(1,1,\dots,1)$
\FOR{$t=1,\dots ,T$}
    \STATE pick random ${\bf x}\in S$
    \STATE compute $nearmiss({\bf x})$ with respect to $S\setminus {\bf x}$
    \STATE compute $nearhit({\bf x})$ with respect to $S\setminus {\bf x}$
    \FOR{$i = 1,\dots , N$}
	\STATE compute $(\bigtriangledown e({\bf w}))_i$
    \ENDFOR
    \STATE ${\bf w} = {\bf w} + \bigtriangledown e({\bf w})$
\ENDFOR
\STATE ${\bf w} \leftarrow {\bf w}^2 / \|{\bf w}^2\|_\infty$ where $({\bf w}^2)_i := ({\bf w}_i)^2$
\end{algorithmic}
\end{algorithm}

\subsection{\label{sec:feature:featureselect_simba_disscuss}Discussion}
The SIMBA algorithm computes a maximum margin guided feature selection which runs in $\Omega(TNm)$ for $m$ training samples with $N$ features.
The number of needed iterations $T$ depends on the individual problem, but we empirically experienced quite good convergence behavior and
usually set $T<100$.\\


\section{\label{sec:feature:select_data}Data Driven Feature Selection}
\index{Feature Selection}\index{Data driven feature selection}\index{Feature Selection: data driven}
All of the combinatoric methods are actually performing a ``smart'' search for the optimal features (or feature combinations).
No matter how ``smart'' this search may be, it always requires that large quantities of the features in the search space are actually computed.
For features like $2p$-Haar (\ref{sec:feature:2p}) or ${\cal SH}_{phase}$ (\ref{sec:feature:SHphase}) that have only few parameters where the parameter space can be limited 
by a-priori knowledge, these combinatoric methods are quite suitable.\\
However, for features like $np$ (\ref{sec:feature:np}) or $vp$-Haar (\ref{sec:feature:nv}) which have a huge set of parameters, e.g. the infinitely many 
possible combinations of the kernel
points, the combinatoric method are completely infeasible. Thus, especially for those features where a automatic feature selection really 
is needed, the previous methods cannot be applied.\\

We tackle this problem by introducing a novel, feature specific (non-generic) selection algorithm, where we learn the optimal feature
parameters from labeled training data. Hence, this approach is constructive and tries to avoid searching large parameter spaces at all.\\

Throughout the rest of this section we use the $np$-Feature (see chapter \ref{sec:feature:np}) to derive the selection algorithm. However, the same 
method can also be directly applied to $nv$-Features (see chapter \ref{sec:feature:nv}).\\
Let us recall the parameterization of the $np$-Features from (\ref{eq:feature:np_lambda}). Regardless of whether we use the original separable 
formulation (\ref{eq:feature:np_final} ) or the fast kernel (\ref{eq:feature:np_formularfast} ), we need to choose the following parameters 
for each feature:  
\begin{equation}
\Lambda := \big\{\kappa_1, \{\kappa_2,r_2,c_2,\Phi_2,\Theta_2\},\dots,
\{\kappa_n,r_n,c_n,\Phi_n,\Theta_n\}\big\}.
\end{equation}
While the selection of the input channels $c_i$ and a limitation of the radii $r_i$ to reasonable values can be done according to a-priori
knowledge of the problem, we derive two data driven methods for the learning of suitable kernel point positions ($\Phi_i,\Theta_i$) and
the non-linear mappings $\kappa_i$.
\subsection{\label{sec:feature:select_data_points}Learning the Position of the Kernel Points}
Let us start with the more difficult problem, the positioning of the kernel points.
Given the parameterization recalled from figure 
\ref{fig:feature:npparameter}, we need to determine the number of kernel points and their position parameterized in $\Phi_i,\Theta_i$:

\begin{figure}[ht]
\centering
\psfrag{x0}{\footnotesize${\bf x}_0$}
\psfrag{x1}{\footnotesize${\bf x}_1$}
\psfrag{x2}{\footnotesize${\bf x}_2$}
\psfrag{x3}{\footnotesize${\bf x}_3$}
\psfrag{x4}{\footnotesize${\bf x}_4$}
\includegraphics[width=0.3\textwidth]{FIGURES/np_parameter.eps}
\psfrag{phi}{\footnotesize$\Phi$}
\psfrag{theta}{\footnotesize$\Theta$}
\psfrag{radius}{\footnotesize$r$}
\psfrag{xi}{\footnotesize${\bf x}_i$}
\includegraphics[width=0.3\textwidth]{FIGURES/np_parameter2.eps}
\caption[Parameterization of ``n-point'' kernels.]{ Parameterization of n-point kernels. {\bf Left}: The $n$ kernel points are 
parameterized as points on a sphere with exception of  ${\it x_0}$, which is by definition placed in the origin of the local kernel 
support ${\bf x}$.
{\bf Right}: Each kernel point ${\it x_i}\in S[r_i]\left({\bf x}\right)$ is parameterized by its spherical coordinate $
(\Phi_i,\Theta_i)$ and distance to the origin (= radius of the sphere) $r_i$.}
\end{figure}

Recall that $np$-Features (see chapter \ref{sec:feature:np}) are
designed to be quite specific features which should detect certain structures. Hence, the kernel points have to be selected such that
the structure of the target objects is reflected in the kernel constellation. We derive the final algorithm in a constructive manner:\\

\paragraph{Step 1: Clustering:} We begin by applying an unsupervised clustering (see \ref{sec:learning:learning}), by applying the $k$-Means algorithm on the labeled training 
data. We utilize the maximum of the simultaneous fast correlation (see section \ref{sec:feature:ncrosscorr}) over several radii of the local harmonic expansions 
of the training data as distance measure for the clustering.\\
After clustering, we use the labels of the training data to select homogeneous clusters, i.e. clusters which are mostly containing members of the target classes.
The number of the selected clusters reflects the number of proposed features. Hence, we tune the clustering such that it
returns the number of desired clusters. We then construct a feature for each of these selected clusters. Figure 
\ref{fig_feature:select_npcluster} shows an example for the clustering step. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{FIGURES/selection_cluster.eps}
\caption[Clustering for the $np$ feature selection.]{\label{fig_feature:select_npcluster} Step 1: sample result of the clustering for the 
$np$-Feature selection on neuronal spine data (see section \ref{sec:app:spine}). The voxel-wise clustering was performed with $k=30$ k-Means 
using the fast correlation over several concentric radii at once.}
\end{figure}

\paragraph{Step 2: Registration of the Cluster Members:} For each of the selected clusters from step 1, we take the centroid of this cluster as
reference and un-rotate all other cluster members according to the results form the correlation (see section \ref{sec:feature:recrotparams}. This way we obtain
a registration of all cluster members. Figure \ref{fig_feature:select_npclusterrot} illustrates\footnote{Thanks to A. Streicher for the Matlab visualization tool.}{} this step for a toy example.

\begin{figure}[ht]
\centering
\psfrag{s1}{$s_1$}
\psfrag{s2}{$s_2$}
\psfrag{sn}{$s_n$}
\psfrag{center}{centroid}
\psfrag{register}{register}
\includegraphics[width=0.8\textwidth]{FIGURES/selection_rot.eps}
\caption[Registration of the Cluster Members for $np$ feature selection.]{\label{fig_feature:select_npclusterrot} Step 2 (toy example): 
for each cluster, we register all cluster members $s_1,\dots,s_n$ to the cluster centroid. The red dot marks the position of the maximum 
correlation with the centroid which is obtained from the correlation matrices from step 1.  }
\end{figure}

\paragraph{Step 3: Construction of the Cluster Representative:} Next, we transform all aligned cluster members back to the spatial domain. 
Hence, we obtain a discrete 3D volume grid representation of spherical surfaces for each considered radius. Then, we compute the 
voxel-wise variance 
$\sigma(r,\Phi_i,\Theta_i)$ at fixed voxel positions $r,\Phi_i,\Theta_i$ over all cluster members (see figure 
\ref{fig_feature:select_npclustervar}). Finally, we locate regions on the surfaces which have a locally stable low variance and the same 
number of regions with a high variance.

\begin{figure}[ht]
\centering
\psfrag{cluster members}{cluster members}
\psfrag{cluster representative}{cluster representative}
\psfrag{high variance}{high variance}
\psfrag{low variance}{low variance}
\includegraphics[width=0.8\textwidth]{FIGURES/selection_var.eps}
\caption[Computing the local variance of the Cluster Members for $np$ feature selection.]{\label{fig_feature:select_npclustervar} 
Step 3 (toy example): generation of the cluster representative. We compute the variance for each discrete position $r,\Phi_i,\Theta_i$
over all registered cluster members. Voxels with a low variance (an example for such a voxel is marked in green) are mapped to the 
representative while voxels with a high variance (an example for such a voxel is marked in red) are set to zero.}
\end{figure}

\paragraph{Step 4: Placing the Kernel Points:} In the last step, we place the kernel points at the regions of low variance (see figure
\ref{fig_feature:select_npclusterpoint}).
Hence, we obtain
the number of needed kernel points, as well as the corresponding parameters $r_i, \Phi_i$ and $\Theta_i$. The regions with high variance are
needed later on for the learning of the non-linear mappings.

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth]{FIGURES/selection_points.eps}
\caption[Placing of the kernel points for $np$ feature selection.]{\label{fig_feature:select_npclusterpoint}
Step 4 (toy example): placing of the kernel points at regions of low variance. }
\end{figure}

An overview of the entire procedure is given in algorithm \ref{algo:feature:select_np_poss}. Placing the kernel points in positions
of low variance guaranties that the points are actually sensing information which is stable and representative for the cluster while
neglecting noise. Since we required that the cluster member have to belong to the same class, the correlation based clustering ensures
that the selected points are discriminative.\\
The usage of the unsupervised clustering enables us to uncover the different types of appearance within the variation of a class. 

\begin{algorithm}
\caption{Feature selection: $np$ kernel point positions}
\label{algo:feature:select_np_poss}
\begin{algorithmic}
\STATE cluster the labeled input data
\STATE select clusters mostly containing the target or background class
\FORALL{clusters}
    \STATE register the cluster members
    \STATE transform cluster members to spatial domain
    \STATE compute voxel-wise variance 
    \STATE place kernel points in regions of low variance
    \STATE obtain $r_i, \Phi_i$ and $\Theta_i$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{\label{sec:feature:select_mapping}Learning the Non-Linear Kernel Mappings}
After selecting the positions for the kernel points, we still need the associated non-linear mappings $\kappa_i$. This problem appears
to be non-trivial, because searching for suitable functions is a variational problem which tend be very difficult to solve.
To overcome these difficulties, we turn to well known regression algorithms which describe the variational problem in terms of easier to
handle parameter optimization problems.\\
For our case, we recall that it is feasible enough to draw the mappings $\kappa_i$ from a rather small set of very simple
but essentially non-linear functions, i.e. functions like $\kappa_1({\it x}_1) = {\it x}_1^2, \kappa_2({\it x}_2) = {\it x}_2^3, \kappa_3({\it x}_3)
= {\it x}_3^4,\dots, \kappa_n({\it x}_4) = \sqrt({\it x}_4), \dots$. Hence, the parameters are the weights of the given mappings. They
can be found by a combinatoric search using MMD or SIMBA.\\

For each feature, we return to the corresponding registered cluster, where we collect the data from the $n$ kernel points as positive labeled
training samples $({\bf x}_i, y_i)$ for the $i$-th cluster member and assign $y_i=1$. The entries of ${\bf x}_i$ are given by the gray-values
at the kernel points.\\
Additionally, we generate the same number of negative training samples from the cluster members by rotating the kernel such that random 
kernel points are positioned in also randomly selected regions with high variance. We label these samples by $y_i=-1$. 
All $x_i$ training samples are combined row-wise in the matrix $X$ and the labels are stored in the vector $Y$.\\

Using $X$, we then construct the matrix ${K}$ containing all possible combinations of the non-linear mappings $\kappa_i$: 
Given $n$ points and $m$ possible non-linear mappings, each row ${ K}_i$ holds  a possible assignment of the $\kappa_i$.
Without loss of generality, we assume $m=n$. Hence, $K$ contains all possible permutations of the $\kappa_i$ assignments to the kernel points
${\bf x}_i$:
\begin{eqnarray}
{\bf K}_i &:=& \left(\kappa_1\big({\bf x}_1\big)\cdot\kappa_2\big({\bf x}_2\big)\cdot\dots\cdot\kappa_n\big({\bf x}_n\big)\right.,\\
&& \dots,\nonumber\\
&&\left. \kappa_n\big({\bf x}_1\big)\cdot\kappa_{n-1}\big({\bf x}_2\big)\cdot\dots\cdot\kappa_1\big({\bf x}_n\big)\right).
\end{eqnarray}

Then we apply the fast MMD algorithm (see section \ref{sec:feature:featureselect_mmd}) on $K$ to find the best combination of the mapping 
given $Y$. The ranking that is returned by MMD then indicates which feature combination is most suitable. At this point we can then
decide to select one or more features with the same kernel constellation but different non-linear mappings from each cluster.




